Equilibrium Selection in Information Elicitation without Verification via Information Monotonicity

Peer-prediction is a mechanism which elicits privately-held, non-variable information from self-interested agents---formally, truth-telling is a strict Bayes Nash equilibrium of the mechanism. The original Peer-prediction mechanism suffers from two main limitations: (1) the mechanism must know the "common prior" of agents' signals; (2) additional undesirable and non-truthful equilibria exist which often have a greater expected payoff than the truth-telling equilibrium. A series of results has successfully weakened the known common prior assumption. However, the equilibrium multiplicity issue remains a challenge. In this paper, we address the above two problems. In the setting where a common prior exists but is not known to the mechanism we show (1) a general negative result applying to a large class of mechanisms showing truth-telling can never pay strictly more in expectation than a particular set of equilibria where agents collude to "relabel" the signals and tell the truth after relabeling signals; (2) provide a mechanism that has no information about the common prior but where truth-telling pays as much in expectation as any relabeling equilibrium and pays strictly more than any other symmetric equilibrium; (3) moreover in our mechanism, if the number of agents is sufficiently large, truth-telling pays similarly to any equilibrium close to a "relabeling" equilibrium and pays strictly more than any equilibrium that is not close to a relabeling equilibrium.

==> additional_explanation.tex <==



In this section, we will see for a specific family of mechanisms $\mathcal{F}$, for any $\mathcal{M}\in \mathcal{F}$, we can use our technique to modify $\mathcal{M}$ to a new mechanism $\mathcal{M}+$ that has truth-telling as \emph{weakly-quasi-focal}. 




Falting\cite{radanovic2013robust} defines a \emph{decomposable} payment scheme (mechanism) as a payment scheme where each agent $i$'s total score his information score plus his prediction score and the information score does not depend on the agent's prediction report and the prediction score does not depend on the agent's information report (signal). Now we consider a family $\mathcal{F}$ of truthful mechanisms where (1) agents are asked to report his signal and prediction over other agents' reported signals; (2) the payment scheme is decomposable; (3) the prediction score for each agent $i$ is $PS(\hat{\sigma},\mathbf{p}_i)$ where $PS(\cdot,\cdot)$ is a strict proper scoring rule and $\mathbf{p}_i$ is agent $i$'s reported prediction. We will show if a truthful mechanism satisfies the above three conditions, then we can modify it to a mechanism that has truth-telling as \emph{weakly-quasi-focal}. 


For any $DPS(PS(\cdot,\cdot))\in \mathcal{F}$, we use the same idea of designing our \emph{Disagreement Mechanism} to modify $DPS$: (a) divide agents into two non-empty groups to create a zero-sum game which has the same equilibria with $DPS$; (b) pay each agent $i$ an extra score that only depends on other agents. We will see this modified $DPS$ has truth-telling as \emph{weakly-quasi-focal} as well. 


For each agent $i$, we define $payment_{DPS(PS(\cdot,\cdot))}(i,\mathbf{r})$ as the payment of agent $i$ given the report profiles of all agents is $\mathbf{r}$ under $DPS$ payment scheme. 

\paragraph{Modified DPS $\mathcal{DPS+}(PS(\cdot,\cdot))$}
\begin{enumerate}
\item Divide the agents into two non-empty groups-group A and group B. For group A, each agent $i_A$ receives a $$ score_{DPS}(i_A,\mathbf{r}) = payment_{DPS(PS(\cdot,\cdot))}(i_A,\mathbf{r})-\frac{1}{|A|}\sum_{j_B\in B} payment_{DPS(PS(\cdot,\cdot))}(j_B,\mathbf{r}) $$ For agents in group B, we use the same way to score them.  
\item Each agent $i$ is matched with two random agents $j,k$, the payment for agent $i$ is 
$$payment_{\mathcal{DPS+}(PS(\cdot,\cdot))}(i,\mathbf{r})=score_{DPS}(i,\mathbf{r})+score_C(r_j,r_k) $$
where $$score_C(r_j,r_k)=\left\{
\begin{aligned}
D^*(\mathbf{\hat{p}}_j,\mathbf{\hat{p}}_k) &  & \hat{\sigma}_j \neq \hat{\sigma}_k \\
-\sqrt{D^*(\mathbf{\hat{p}}_j,\mathbf{\hat{p}}_k)} &  & \hat{\sigma}_j = \hat{\sigma}_k 
\end{aligned}\right.
$$
\end{enumerate}


\begin{theorem}[Main Theorem]
Given any symmetric, non-zero, informative, fine-grained and ensemble prior, if the number of agents $n\geq 3$, $DPS+(PS(\cdot,\cdot))$ has truth-telling as a \emph{$(\tau_1,\tau_2,\gamma_1,\gamma_2)$-weakly-quasi-focal} equilibrium with $\tau_1(\gamma_1)=O(\sqrt[3]{\gamma_1})$, $\gamma_2(n)=O(\frac{m}{\sqrt{n}})$ and $\tau_2(n)=O(\sqrt[6]{\frac{m^2}{n})}$ (the constants we omit only depend on the first two moments of prior $Q$),
where $m$ is the number of signals, $n$ is the number of agents, and actually $\tau_1(\gamma_1)=\frac{1}{c_1}\sqrt[3]{\frac{\gamma_1}{c_2,c_3,c_4}}$, $\gamma_2(n)=\frac{4\sqrt{2}m}{\sqrt{n}}$ and $\tau_2^6(n)=\frac{128*m^2}{n c_1^6 (c_2 c_3 c_4)^2}$, $c_1 = \min_{s,t\in \Sigma} q(s|t)$, $c_2 = \min_{s,t\in \Sigma}Pr(s,t)$, $c_3 = \min_{u,v} \max_{s,t}||\frac{q(u|s)}{q(u|t)}-\frac{q(v|s)}{q(v|t)}||^2$, $c_4 = \min_{s,t,u} f''(\frac{q(u|s)}{q(u|t)})$ where $f(x)=(\sqrt{x}-1)^2$. 
 
\end{theorem}

\begin{proof}
Since $DPS$ is decomposable, for each agent $i$, his information score does not depend on his prediction which implies that his best response for prediction only needs to maximize his prediction score. Based on Claim~\ref{claim:best prediction} and the property of strict proper scoring rule, his best response for prediction would be $\theta_{-i} \mathbf{q}_{\sigma_i}$ (his belief for the likelihood of other agents' reported signals) given his private signal is $\sigma_i$. So at any equilibrium $s$ under $DPS$, we have $s=s_{BP}$ which implies $\textit{ClassificationScore}(s)= \textit{TotalDivergence}(s_{BP})$ in $DPS$. So our main lemma still holds, then the rest of the proof follows from our previous proof for our main theorem. 


\end{proof}






%We call \emph{information-prediction} mechanisms as a family of \emph{truthful} mechanisms where agents are asked to report both his signal and prediction, and paid ``information score'' plus ``prediction score'' where the ``prediction score'' of each agent is maximized if and only if his prediction is the likelihood of other agents' reported signals. 


%In our \emph{Disagreement Mechanism}, each agent's information score depends both on his reported signal and prediction. So the equilibrium analysis here is complicated. However, for the \emph{information-prediction} mechanism where each agent's information score only depends his reported signal and other agents' report profiles, at any equilibrium, for any $i$, agent $i$'s prediction must be $\theta_{-i} \mathbf{q}_{\sigma_i}$ (his belief for the likelihood of other agents' reported signals) given his private signal is $\sigma_i$ since ``prediction score'' is the only part in agent $i$'s payment that relates to agent $i$'s prediction. For these kind of mechanisms, our techniques can be applied directly by making a new mechanism with zero-sum payment that has the same equilibria with the original mechanism and then pay each agent $i$ an extra score which is $D_f(\hat{\mathbf{q}}_j,\hat{\mathbf{q}}_k)$ where $D_f$ is a $f$-divergence and $\hat{\mathbf{q}}_j,\hat{\mathbf{q}}_k$ are agent $j,k$'s reported predictions respectively. Note that by information monotoncity, given SNIFE prior $Q$, if agents play symmetric strategy, the agents-welfare of the new mechanism will be maximized only if agents play permutation strategy profiles. Actually, by the same proof we have, for this new mechanism, truth-telling is \emph{weakly-quasi-focal}. 

The multi-RBTS mechanism in \cite{radanovic2013robust} is in $\mathcal{F}$, the modified multi-RBTS mechanism has truth-telling as \emph{weakly-quasi-focal} while this mechanism requires additional assumption (self-predicting assumption\cite{radanovic2013robust}: any agent $i$ will believe another agent $k$ is most likely to observe a certain value x when she herself also observes this value) for prior to make truth-telling an equilibrium and our \emph{Disagreement Mechanism} does not need this additional assumption. 
